DART: Implicit Doppler Tomography for Radar Novel View Synthesis

Simulation is an invaluable tool for radio-frequency system designers that enables rapid prototyping of various algorithms for imaging, target detection, classification, and tracking. However, simulating realistic radar scans is a challenging task that requires an accurate model of the scene, radio frequency material properties, and a corresponding radar synthesis function. Rather than specifying these models explicitly, we propose DART - Doppler Aided Radar Tomography, a Neural Radiance Field-inspired method which uses radar-specific physics to create a reflectance and transmittance-based rendering pipeline for range-Doppler images. We then evaluate DART by constructing a custom data collection platform and collecting a novel radar dataset together with accurate position and instantaneous velocity measurements from lidar-based localization. In comparison to state-of-the-art baselines, DART synthesizes superior radar range-Doppler images from novel views across all datasets and additionally can be used to generate high quality tomographic images.

==> figure-blocks/failures.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/examples-failure.pdf}
\vspace{-2.5em}
\caption{Range-Doppler (with range on the y-axis) plots of two example failure cases for our method.}
\vspace{-1em}
\label{fig:failures}
\end{figure*}

==> figure-blocks/imaging.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/car.pdf}
\vspace{-3em}
\caption{Imaging a car using LIDAR, our method, and incoherent SAR with 20cm and 4cm grids, showing 2D slices of the sampled radar volume along the vertical and horizontal axis. While  SAR with a coarse grid creates a blurry image, and SAR with a fine grid creates a noisy image, DART is able to clearly resolve the car.}
\vspace{-1em}
\label{fig:image-car}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/tent.pdf}
\vspace{-3em}
\caption{Imaging a tent with a metal filing cabinet hidden inside (the tent is fully zipped up during data collection), again shown as slices along the vertical and horizontal axis. While LIDAR cannot see through the tent, radar can clearly see a reflective object at the center of the tent, in addition to resolving the structure of the metal tent poles.}
\label{fig:image-tent}
\vspace{-1em}
\end{figure*}


==> figure-blocks/lidar.tex <==
\begin{figure*}
\centering
\begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[height=0.6\textwidth]{figures/cichallway-lidar.pdf}
    \vspace{-0.5em}
    \caption{Hall A \& Hall B}
\end{subfigure}
\begin{subfigure}[b]{0.144\textwidth}
    \centering
    \includegraphics[height=\textwidth]{figures/arena-lidar.pdf}
    \vspace{-0.5em}
    \caption{Lab}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[height=0.6\textwidth]{figures/arena-plus-lidar.pdf}
    \vspace{-0.5em}
    \caption{Lab+}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[height=0.6\textwidth]{figures/cafe-lidar.pdf}
    \vspace{-0.5em}
    \caption{Cafe}
\end{subfigure}
\vspace{-1em}
\caption{Lidar maps (across a horizontal slice) created by Cartographer along with the trajectory taken; two separate trajectories were taken for Hall A and Hall B.}
\vspace*{-1em}
\label{fig:lidar}
\end{figure*}

